Bayesian Confidence Calibration for Epistemic Uncertainty Modelling

Modern neural networks have found to be miscalibrated in terms of confidence calibration, i.e., their predicted confidence scores do not reflect the observed accuracy or precision. Recent work has introduced methods for post-hoc confidence calibration for classification as well as for object detection to address this issue. Especially in safety critical applications, it is crucial to obtain a reliable self-assessment of a model. But what if the calibration method itself is uncertain, e.g., due to an insufficient knowledge base? We introduce Bayesian confidence calibration - a framework to obtain calibrated confidence estimates in conjunction with an uncertainty of the calibration method. Commonly, Bayesian neural networks (BNN) are used to indicate a network's uncertainty about a certain prediction. BNNs are interpreted as neural networks that use distributions instead of weights for inference. We transfer this idea of using distributions to confidence calibration. For this purpose, we use stochastic variational inference to build a calibration mapping that outputs a probability distribution rather than a single calibrated estimate. Using this approach, we achieve state-of-the-art calibration performance for object detection calibration. Finally, we show that this additional type of uncertainty can be used as a sufficient criterion for covariate shift detection. All code is open source and available at https://github.com/EFS-OpenSource/calibration-framework.

==> evaluation/cityscapes-on-cityscapes-Cityscapes-mask-rcnn-iou-0.50-MPIW.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
LC &   6.461 &  16.969 &  16.762 &  22.783 \\
BC &   7.083 &  16.207 &  18.869 &  22.217 \\
\bottomrule
\end{tabular}


==> evaluation/cityscapes-on-cityscapes-Cityscapes-mask-rcnn-iou-0.50-PICP.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
LC &  89.062 &  89.560 &  92.652 &  84.600 \\
BC &  74.678 &  91.162 &  93.628 &  85.545 \\
\bottomrule
\end{tabular}


==> evaluation/cityscapes-on-cityscapes-Cityscapes-mask-rcnn-iou-0.75-MPIW.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
LC &   7.664 &  20.202 &  19.624 &  28.443 \\
BC &   6.901 &  19.660 &  21.642 &  25.141 \\
\bottomrule
\end{tabular}


==> evaluation/cityscapes-on-cityscapes-Cityscapes-mask-rcnn-iou-0.75-PICP.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
LC &  98.848 &  99.135 &  99.217 &  98.576 \\
BC &  95.166 &  99.110 &  99.315 &  98.321 \\
\bottomrule
\end{tabular}


==> evaluation/cityscapes-on-mscoco-Cityscapes-mask-rcnn-iou-0.50-ECE.tex <==
\begin{tabular}{lllll}
\toprule
{} &        $(\pred)$ &         $(\pred, \centerx, \centery)$ &            $(\pred, \width, \height)$ &           full \\
\midrule
baseline &        10.928 &         11.935 &          11.009 &         11.008 \\
HB       &         6.131 &          8.578 &           8.367 &          9.821 \\
LC       &  5.361 $+$0.061 &  10.876 $-$1.387 &  16.739 $-$10.605 &  10.258 $-$0.582 \\
BC       &  5.354 $+$3.107 &   8.640 $+$0.234 &    9.599 $+$1.184 &   9.051 $+$2.414 \\
\bottomrule
\end{tabular}


==> evaluation/cityscapes-on-mscoco-Cityscapes-mask-rcnn-iou-0.50-MPIW.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
LC &   6.722 &  44.671 &  31.782 &  65.994 \\
BC &   8.055 &  22.625 &  19.929 &  25.188 \\
\bottomrule
\end{tabular}


==> evaluation/cityscapes-on-mscoco-Cityscapes-mask-rcnn-iou-0.50-PICP-MPIW.tex <==
\begin{tabular}{llrrrr}
\toprule
     &    &  $(\pred)$ &  $\pred, (\centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
\multirow{2}{*}{PICP} & LC &  90.993 &  98.190 &  91.684 &  99.073 \\
     & BC &  82.595 &  92.108 &  92.882 &  88.055 \\
\cline{1-6}
\multirow{2}{*}{MPIW} & LC &   6.722 &  44.671 &  31.782 &  65.994 \\
     & BC &   8.055 &  22.625 &  19.929 &  25.188 \\
\bottomrule
\end{tabular}


==> evaluation/cityscapes-on-mscoco-Cityscapes-mask-rcnn-iou-0.50-PICP.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
LC &  90.993 &  98.190 &  91.684 &  99.073 \\
BC &  82.595 &  92.108 &  92.882 &  88.055 \\
\bottomrule
\end{tabular}


==> evaluation/cityscapes-on-mscoco-Cityscapes-mask-rcnn-iou-0.75-ECE.tex <==
\begin{tabular}{lllll}
\toprule
{} &         $(\pred)$ &         $(\pred, \centerx, \centery)$ &            $(\pred, \width, \height)$ &           full \\
\midrule
baseline &         22.792 &         23.646 &          22.369 &         21.664 \\
HB       &         10.263 &         14.028 &          13.637 &         17.325 \\
LC       &  11.782 $-$0.016 &  17.587 $-$5.317 &  23.979 $-$11.193 &  17.809 $-$5.823 \\
BC       &  12.097 $+$6.206 &  15.537 $+$0.238 &   10.289 $+$5.435 &  14.341 $+$2.662 \\
\bottomrule
\end{tabular}


==> evaluation/cityscapes-on-mscoco-Cityscapes-mask-rcnn-iou-0.75-MPIW.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
LC &   6.633 &  44.186 &  39.461 &  65.893 \\
BC &   6.966 &  21.667 &  18.955 &  23.835 \\
\bottomrule
\end{tabular}


==> evaluation/cityscapes-on-mscoco-Cityscapes-mask-rcnn-iou-0.75-PICP-MPIW.tex <==
\begin{tabular}{llrrrr}
\toprule
     &    &  $(\pred)$ &  $\pred, (\centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
\multirow{2}{*}{PICP} & LC &  95.601 &  99.434 &  99.949 &  99.740 \\
     & BC &  93.192 &  99.003 &  99.561 &  96.490 \\
\cline{1-6}
\multirow{2}{*}{MPIW} & LC &   6.633 &  44.186 &  39.461 &  65.893 \\
     & BC &   6.966 &  21.667 &  18.955 &  23.835 \\
\bottomrule
\end{tabular}


==> evaluation/cityscapes-on-mscoco-Cityscapes-mask-rcnn-iou-0.75-PICP.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &   full \\
\midrule
LC &  95.601 &  99.434 &  99.949 &  99.74 \\
BC &  93.192 &  99.003 &  99.561 &  96.49 \\
\bottomrule
\end{tabular}


==> evaluation/mscoco-on-cityscapes-COCO-faster-rcnn-iou-0.50-ECE.tex <==
\begin{tabular}{lllll}
\toprule
{} &         $(\pred)$ &         $(\pred, \centerx, \centery)$ &           $(\pred, \width, \height)$ &           full \\
\midrule
baseline &         15.077 &         15.165 &         14.677 &         14.839 \\
HB       &         13.418 &         14.046 &         14.051 &         12.739 \\
LC       &  13.198 $+$0.040 &  13.631 $-$0.123 &  16.523 $-$1.884 &  17.004 $-$2.103 \\
BC       &  13.164 $+$0.513 &  13.311 $-$0.413 &  14.740 $+$1.848 &  15.382 $-$1.115 \\
\bottomrule
\end{tabular}


==> evaluation/mscoco-on-cityscapes-COCO-faster-rcnn-iou-0.50-MPIW.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
LC &   5.976 &  13.332 &  14.319 &  17.627 \\
BC &   7.269 &  16.617 &  17.686 &  20.275 \\
\bottomrule
\end{tabular}


==> evaluation/mscoco-on-cityscapes-COCO-faster-rcnn-iou-0.50-PICP-MPIW.tex <==
\begin{tabular}{llrrrr}
\toprule
     &    &  $(\pred)$ &  $\pred, (\centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
\multirow{2}{*}{PICP} & LC &  92.960 &  83.892 &  90.128 &  79.391 \\
     & BC &  85.887 &  89.222 &  93.153 &  82.843 \\
\cline{1-6}
\multirow{2}{*}{MPIW} & LC &   5.976 &  13.332 &  14.319 &  17.627 \\
     & BC &   7.269 &  16.617 &  17.686 &  20.275 \\
\bottomrule
\end{tabular}


==> evaluation/mscoco-on-cityscapes-COCO-faster-rcnn-iou-0.50-PICP.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
LC &  92.960 &  83.892 &  90.128 &  79.391 \\
BC &  85.887 &  89.222 &  93.153 &  82.843 \\
\bottomrule
\end{tabular}


==> evaluation/mscoco-on-cityscapes-COCO-faster-rcnn-iou-0.75-ECE.tex <==
\begin{tabular}{lllll}
\toprule
{} &         $(\pred)$ &         $(\pred, \centerx, \centery)$ &           $(\pred, \width, \height)$ &           full \\
\midrule
baseline &         34.534 &         32.525 &         34.228 &         33.710 \\
HB       &         22.250 &         22.068 &         21.375 &         19.811 \\
LC       &  21.656 $-$0.590 &  20.880 $+$0.815 &  25.108 $-$1.596 &  24.848 $-$2.907 \\
BC       &  21.530 $-$0.324 &  20.588 $+$1.764 &  21.545 $+$3.504 &  22.324 $+$1.570 \\
\bottomrule
\end{tabular}


==> evaluation/mscoco-on-cityscapes-COCO-faster-rcnn-iou-0.75-MPIW.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
LC &    7.24 &  16.624 &  16.435 &  23.549 \\
BC &    8.02 &  18.683 &  23.152 &  26.088 \\
\bottomrule
\end{tabular}


==> evaluation/mscoco-on-cityscapes-COCO-faster-rcnn-iou-0.75-PICP-MPIW.tex <==
\begin{tabular}{llrrrr}
\toprule
     &    &  $(\pred)$ &  $\pred, (\centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
\multirow{2}{*}{PICP} & LC &  99.413 &  97.776 &  98.446 &  96.990 \\
     & BC &  91.949 &  98.612 &  99.967 &  98.386 \\
\cline{1-6}
\multirow{2}{*}{MPIW} & LC &   7.240 &  16.624 &  16.435 &  23.549 \\
     & BC &   8.020 &  18.683 &  23.152 &  26.088 \\
\bottomrule
\end{tabular}


==> evaluation/mscoco-on-cityscapes-COCO-faster-rcnn-iou-0.75-PICP.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
LC &  99.413 &  97.776 &  98.446 &  96.990 \\
BC &  91.949 &  98.612 &  99.967 &  98.386 \\
\bottomrule
\end{tabular}


==> evaluation/mscoco-on-mscoco-COCO-faster-rcnn-iou-0.50-MPIW.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
LC &   5.763 &  14.793 &  13.458 &  21.248 \\
BC &   7.026 &  15.340 &  16.527 &  20.193 \\
\bottomrule
\end{tabular}


==> evaluation/mscoco-on-mscoco-COCO-faster-rcnn-iou-0.50-PICP.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
LC &  84.719 &  78.326 &  83.471 &  82.217 \\
BC &  79.431 &  80.051 &  84.315 &  80.627 \\
\bottomrule
\end{tabular}


==> evaluation/mscoco-on-mscoco-COCO-faster-rcnn-iou-0.75-MPIW.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
LC &   6.947 &  17.655 &  16.551 &  25.724 \\
BC &   6.979 &  19.120 &  20.172 &  24.721 \\
\bottomrule
\end{tabular}


==> evaluation/mscoco-on-mscoco-COCO-faster-rcnn-iou-0.75-PICP.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &   full \\
\midrule
LC &  99.161 &  95.455 &  96.292 &  96.25 \\
BC &  85.824 &  97.340 &  97.272 &  95.51 \\
\bottomrule
\end{tabular}


==> evaluation/mscoco-on-mscoco-COCO-retinanet-iou-0.50-MPIW.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
LC &   6.324 &  15.187 &  15.501 &  22.334 \\
BC &   8.148 &  17.048 &  15.641 &  19.362 \\
\bottomrule
\end{tabular}


==> evaluation/mscoco-on-mscoco-COCO-retinanet-iou-0.50-PICP.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
LC &  82.237 &  78.886 &  86.076 &  82.712 \\
BC &  80.022 &  77.568 &  75.667 &  72.555 \\
\bottomrule
\end{tabular}


==> evaluation/mscoco-on-mscoco-COCO-retinanet-iou-0.75-MPIW.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
LC &   7.021 &  18.644 &  17.963 &  26.962 \\
BC &   8.954 &  20.124 &  19.458 &  24.093 \\
\bottomrule
\end{tabular}


==> evaluation/mscoco-on-mscoco-COCO-retinanet-iou-0.75-PICP.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  $(\pred)$ &  $(\pred, \centerx, \centery)$ &    $(\pred, \width, \height)$ &    full \\
\midrule
LC &  98.764 &  95.448 &  98.465 &  97.195 \\
BC &  97.404 &  96.206 &  92.324 &  89.598 \\
\bottomrule
\end{tabular}


==> img/miscalibration.tex <==
\begin{figure*}[t]
	\centering
	\begin{overpic}[tics=2, width=1.0\linewidth]{img/miscalibration.png}
		
		% column captions
		\put(3, 62.8){a) Faster R-CNN on MS COCO}
		\put(39, 62.8){b) RetinaNet on MS COCO}
		\put(71, 62.8){c) Mask R-CNN on Cityscapes}
		
		% row captions
		\put(1, 38){\rotatebox{90}{rel. D-ECE @ IoU 0.50}}
		\put(1, 6.5){\rotatebox{90}{rel. D-ECE @ IoU 0.75}}
		
		
		% ------------------------------------------------------- %
		% x-axis ticks
		\put(3.5, 34){\rotatebox{45}{\tiny{HB}}}
		\put(5.4, 34){\rotatebox{45}{\tiny{LC}}}
		\put(7.3, 34){\rotatebox{45}{\tiny{BC}}}
		
		\put(11.2, 34){\rotatebox{45}{\tiny{HB}}}
		\put(13.1, 34){\rotatebox{45}{\tiny{LC}}}
		\put(15, 34){\rotatebox{45}{\tiny{BC}}}
		
		\put(18.8, 34){\rotatebox{45}{\tiny{HB}}}
		\put(20.7, 34){\rotatebox{45}{\tiny{LC}}}
		\put(22.6, 34){\rotatebox{45}{\tiny{BC}}}
		
		\put(26.4, 34){\rotatebox{45}{\tiny{HB}}}
		\put(28.3, 34){\rotatebox{45}{\tiny{LC}}}
		\put(30.2, 34){\rotatebox{45}{\tiny{BC}}}
		
		% ------------------------------ %
		% +33.8
		\put(37.3, 34){\rotatebox{45}{\tiny{HB}}}
		\put(39.2, 34){\rotatebox{45}{\tiny{LC}}}
		\put(41.1, 34){\rotatebox{45}{\tiny{BC}}}
		
		\put(45, 34){\rotatebox{45}{\tiny{HB}}}
		\put(46.9, 34){\rotatebox{45}{\tiny{LC}}}
		\put(48.8, 34){\rotatebox{45}{\tiny{BC}}}
		
		\put(52.6, 34){\rotatebox{45}{\tiny{HB}}}
		\put(54.5, 34){\rotatebox{45}{\tiny{LC}}}
		\put(56.4, 34){\rotatebox{45}{\tiny{BC}}}
		
		\put(60.2, 34){\rotatebox{45}{\tiny{HB}}}
		\put(62.1, 34){\rotatebox{45}{\tiny{LC}}}
		\put(64, 34){\rotatebox{45}{\tiny{BC}}}
		
		% ------------------------------ %
		% +33.8
		\put(71.1, 34){\rotatebox{45}{\tiny{HB}}}
		\put(73, 34){\rotatebox{45}{\tiny{LC}}}
		\put(74.9, 34){\rotatebox{45}{\tiny{BC}}}
		
		\put(78.8, 34){\rotatebox{45}{\tiny{HB}}}
		\put(80.7, 34){\rotatebox{45}{\tiny{LC}}}
		\put(82.6, 34){\rotatebox{45}{\tiny{BC}}}
		
		\put(86.4, 34){\rotatebox{45}{\tiny{HB}}}
		\put(88.3, 34){\rotatebox{45}{\tiny{LC}}}
		\put(90.2, 34){\rotatebox{45}{\tiny{BC}}}
		
		\put(94, 34){\rotatebox{45}{\tiny{HB}}}
		\put(95.9, 34){\rotatebox{45}{\tiny{LC}}}
		\put(97.8, 34){\rotatebox{45}{\tiny{BC}}}
		
		% ------------------------------ %
		% ------------------------------ %
		
		\put(3.5, 2.5){\rotatebox{45}{\tiny{HB}}}
		\put(5.4, 2.5){\rotatebox{45}{\tiny{LC}}}
		\put(7.3, 2.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(11.2, 2.5){\rotatebox{45}{\tiny{HB}}}
		\put(13.1, 2.5){\rotatebox{45}{\tiny{LC}}}
		\put(15, 2.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(18.8, 2.5){\rotatebox{45}{\tiny{HB}}}
		\put(20.7, 2.5){\rotatebox{45}{\tiny{LC}}}
		\put(22.6, 2.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(26.4, 2.5){\rotatebox{45}{\tiny{HB}}}
		\put(28.3, 2.5){\rotatebox{45}{\tiny{LC}}}
		\put(30.2, 2.5){\rotatebox{45}{\tiny{BC}}}
		
		% ------------------------------ %
		% +33.8
		\put(37.3, 2.5){\rotatebox{45}{\tiny{HB}}}
		\put(39.2, 2.5){\rotatebox{45}{\tiny{LC}}}
		\put(41.1, 2.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(45, 2.5){\rotatebox{45}{\tiny{HB}}}
		\put(46.9, 2.5){\rotatebox{45}{\tiny{LC}}}
		\put(48.8, 2.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(52.6, 2.5){\rotatebox{45}{\tiny{HB}}}
		\put(54.5, 2.5){\rotatebox{45}{\tiny{LC}}}
		\put(56.4, 2.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(60.2, 2.5){\rotatebox{45}{\tiny{HB}}}
		\put(62.1, 2.5){\rotatebox{45}{\tiny{LC}}}
		\put(64, 2.5){\rotatebox{45}{\tiny{BC}}}
		
		% ------------------------------ %
		% +33.8
		\put(71.1, 2.5){\rotatebox{45}{\tiny{HB}}}
		\put(73, 2.5){\rotatebox{45}{\tiny{LC}}}
		\put(74.9, 2.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(78.8, 2.5){\rotatebox{45}{\tiny{HB}}}
		\put(80.7, 2.5){\rotatebox{45}{\tiny{LC}}}
		\put(82.6, 2.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(86.4, 2.5){\rotatebox{45}{\tiny{HB}}}
		\put(88.3, 2.5){\rotatebox{45}{\tiny{LC}}}
		\put(90.2, 2.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(94, 2.5){\rotatebox{45}{\tiny{HB}}}
		\put(95.9, 2.5){\rotatebox{45}{\tiny{LC}}}
		\put(97.8, 2.5){\rotatebox{45}{\tiny{BC}}}
		
		% ------------------------------------------------------- %
		% grouping of calibration methods on x-axis via circled digits
		\put(5.9,32.5){\textbf{\tiny\circled{1}}}
		\put(13.6,32.5){\textbf{\tiny\circled{2}}}
		\put(21.15,32.5){\textbf{\tiny\circled{3}}}
		\put(28.65,32.5){\textbf{\tiny\circled{4}}}
		
		% ------------------------------ %
		% +33.8
		\put(39.7,32.5){\textbf{\tiny\circled{1}}}
		\put(47.4,32.5){\textbf{\tiny\circled{2}}}
		\put(54.95,32.5){\textbf{\tiny\circled{3}}}
		\put(62.45,32.5){\textbf{\tiny\circled{4}}}
		
		% ------------------------------ %
		% +33.8
		\put(73.5,32.5){\textbf{\tiny\circled{1}}}
		\put(81.2,32.5){\textbf{\tiny\circled{2}}}
		\put(88.75,32.5){\textbf{\tiny\circled{3}}}
		\put(96.25,32.5){\textbf{\tiny\circled{4}}}
		
		% ------------------------------ %
		% ------------------------------ %
		
		\put(5.9,1){\textbf{\tiny\circled{1}}}
		\put(13.6,1){\textbf{\tiny\circled{2}}}
		\put(21.15,1){\textbf{\tiny\circled{3}}}
		\put(28.65,1){\textbf{\tiny\circled{4}}}
		
		% ------------------------------ %
		% +33.8
		\put(39.7,1){\textbf{\tiny\circled{1}}}
		\put(47.4,1){\textbf{\tiny\circled{2}}}
		\put(54.95,1){\textbf{\tiny\circled{3}}}
		\put(62.45,1){\textbf{\tiny\circled{4}}}
		
		% ------------------------------ %
		% +33.8
		\put(73.5,1){\textbf{\tiny\circled{1}}}
		\put(81.2,1){\textbf{\tiny\circled{2}}}
		\put(88.75,1){\textbf{\tiny\circled{3}}}
		\put(96.25,1){\textbf{\tiny\circled{4}}}
		
		% ------------------------------------------------------- %
		% D-ECE baselines
		\put(5, 60.5){\tiny{5.65\%}}
		\put(12.7,60.5){\tiny{5.83\%}}
		\put(20.3,60.5){\tiny{6.07\%}}
		\put(27.7,60.5){\tiny{6.36\%}}
		
		% ------------------------------ %
		% +33.8
		
		\put(38.8, 60.5){\tiny{13.67\%}}
		\put(46.5,60.5){\tiny{12.47\%}}
		\put(54.1,60.5){\tiny{15.82\%}}
		\put(61.2,60.5){\tiny{13.45\%}}
		
		% ------------------------------ %
		% +33.8
		
		\put(72.6, 60.5){\tiny{10.50\%}}
		\put(80.3,60.5){\tiny{8.66\%}}
		\put(87.9,60.5){\tiny{9.84\%}}
		\put(95.7,60.5){\tiny{9.97\%}}
		
		% ------------------------------ %
		% ------------------------------ %
		
		\put(5, 29){\tiny{13.30\%}}
		\put(12.7,29){\tiny{12.66\%}}
		\put(20.3,29){\tiny{12.74\%}}
		\put(27.3,29){\tiny{12.40\%}}
		
		% ------------------------------ %
		% +33.8
		
		\put(38.8, 29){\tiny{2.99\%}}
		\put(46.5,29){\tiny{7.94\%}}
		\put(54.1,29){\tiny{8.27\%}}
		\put(61.9,29){\tiny{7.25\%}}
		
		% ------------------------------ %
		% +33.8
		
		\put(72.6, 29){\tiny{30.10\%}}
		\put(80.3,29){\tiny{24.07\%}}
		\put(87.9,29){\tiny{29.19\%}}
		\put(95.2,29){\tiny{27.94\%}}
		
		
		% ------------------------------------------------------- %
		% D-ECE detailled
		\put(4.5, 37){\rotatebox{90}{\color{white}\tiny{$1.44\%$}}}
		\put(6.4125, 37){\rotatebox{90}{\color{white}\tiny{$1.95\%$}}}
		\put(8.25, 37){\rotatebox{90}{\color{white}\tiny{$1.58\%$}}}
		
		\put(6.4125, 47){\rotatebox{90}{\color{black}\tiny{$+0.09\%$}}}
		\put(8.25, 47){\rotatebox{90}{\color{black}\tiny{$+0.77\%$}}}
		
		
		\put(12.2, 37){\rotatebox{90}{\color{white}\tiny{$5.64\%$}}}
		\put(14.1125, 37){\rotatebox{90}{\color{white}\tiny{$5.69\% - 0.01\%$}}}
		\put(15.95, 37){\rotatebox{90}{\color{white}\tiny{$5.69\% + 0.16\%$}}}
		
		\put(19.7, 37){\rotatebox{90}{\color{white}\tiny{$2.68\%$}}}
		\put(21.6125, 37){\rotatebox{90}{\color{white}\tiny{$2.32\%$}}}
		\put(23.45, 37){\rotatebox{90}{\color{white}\tiny{$2.37\%$}}}
		
		\put(21.6125, 47){\rotatebox{90}{\color{black}\tiny{$+0.19\%$}}}
		\put(23.45, 47){\rotatebox{90}{\color{black}\tiny{$+0.22\%$}}}
		
		\put(27.2, 37){\rotatebox{90}{\color{white}\tiny{$4.74\%$}}}
		\put(29.1125, 37){\rotatebox{90}{\color{white}\tiny{$4.15\% + 0.13\%$}}}
		\put(30.95, 37){\rotatebox{90}{\color{white}\tiny{$4.25\% + 0.16\%$}}}
		
		% ------------------------------ %
		% +33.8
		\put(38.3, 41){\rotatebox{90}{\color{black}\tiny{$1.53\%$}}}
		\put(40.2125, 41){\rotatebox{90}{\color{black}\tiny{$2.00\% + 0.03$}}}
		\put(42.05, 41){\rotatebox{90}{\color{black}\tiny{$1.53\% - 0.05$}}}
		
		\put(46, 37){\rotatebox{90}{\color{white}\tiny{$6.14\%$}}}
		\put(47.9125, 37){\rotatebox{90}{\color{white}\tiny{$6.15\% - 0.06\%$}}}
		\put(49.75, 37){\rotatebox{90}{\color{white}\tiny{$6.33\% + 0.07\%$}}}
		
		\put(53.5, 37){\rotatebox{90}{\color{white}\tiny{$3.33\%$}}}
		\put(55.4125, 37){\rotatebox{90}{\color{white}\tiny{$3.15\%$}}}
		\put(57.25, 37){\rotatebox{90}{\color{white}\tiny{$2.99\%$}}}
		
		\put(55.4125, 43){\rotatebox{90}{\color{black}\tiny{$+0.06\%$}}}
		\put(57.25, 43){\rotatebox{90}{\color{black}\tiny{$+0.18\%$}}}
		
		\put(61, 37){\rotatebox{90}{\color{white}\tiny{$4.59\%$}}}
		\put(62.9125, 37){\rotatebox{90}{\color{white}\tiny{$4.12\%$}}}
		\put(64.75, 37){\rotatebox{90}{\color{white}\tiny{$4.71\%$}}}
		
		\put(62.9125, 46){\rotatebox{90}{\color{black}\tiny{$+0.29\%$}}}
		\put(64.75, 46){\rotatebox{90}{\color{black}\tiny{$-0.42\%$}}}
		
		% ------------------------------ %
		% +33.8
		\put(72.1, 37){\rotatebox{90}{\color{white}\tiny{$3.02\%$}}}
		\put(74.0125, 37){\rotatebox{90}{\color{white}\tiny{$3.42\%$}}}
		\put(75.85, 37){\rotatebox{90}{\color{white}\tiny{$3.57\%$}}}
		
		\put(74.0125, 48){\rotatebox{90}{\color{black}\tiny{$+ 0.15\%$}}}
		\put(75.85, 48){\rotatebox{90}{\color{black}\tiny{$+ 1.16\%$}}}
		
		\put(79.8, 37){\rotatebox{90}{\color{white}\tiny{$4.50\%$}}}
		\put(81.7125, 37){\rotatebox{90}{\color{white}\tiny{$4.32\% + 0.56\%$}}}
		\put(83.55, 37){\rotatebox{90}{\color{white}\tiny{$4.67\% - 0.07\%$}}}
		
		\put(87.3, 37){\rotatebox{90}{\color{white}\tiny{$3.16\%$}}}
		\put(89.2125, 37){\rotatebox{90}{\color{white}\tiny{$2.37\%$}}}
		\put(91.05, 37){\rotatebox{90}{\color{white}\tiny{$2.69\%$}}}
		
		\put(89.2125, 46){\rotatebox{90}{\color{black}\tiny{$+1.36\%$}}}
		\put(91.05, 46){\rotatebox{90}{\color{black}\tiny{$+0.52\%$}}}
		
		\put(94.9, 37){\rotatebox{90}{\color{white}\tiny{$5.37\%$}}}
		\put(96.7125, 37){\rotatebox{90}{\color{white}\tiny{$4.94\% + 0.66\%$}}}
		\put(98.55, 37){\rotatebox{90}{\color{white}\tiny{$5.35\% + 0.22\%$}}}
		
		% ------------------------------ %
		% ------------------------------ %
		
		\put(4.5, 8){\rotatebox{90}{\color{black}\tiny{$1.47\%$}}}
		\put(6.4125, 5.5){\rotatebox{90}{\color{white}\tiny{$2.97\%$}}}
		\put(8.25, 5.5){\rotatebox{90}{\color{white}\tiny{$2.36\%$}}}
		
		\put(6.4125, 11){\rotatebox{90}{\color{black}\tiny{$+0.09\%$}}}
		\put(8.25, 11){\rotatebox{90}{\color{black}\tiny{$+6.10\%$}}}
		
		
		\put(12.2, 5.5){\rotatebox{90}{\color{white}\tiny{$6.61\%$}}}
		\put(14.1125, 5.5){\rotatebox{90}{\color{white}\tiny{$7.02\% - 0.40\%$}}}
		\put(15.95, 5.5){\rotatebox{90}{\color{white}\tiny{$7.12\% + 0.19\%$}}}
		
		\put(19.7, 5.5){\rotatebox{90}{\color{white}\tiny{$3.66\%$}}}
		\put(21.6125, 5.5){\rotatebox{90}{\color{white}\tiny{$3.68\%$}}}
		\put(23.45, 5.5){\rotatebox{90}{\color{white}\tiny{$3.36\%$}}}
		
		\put(21.6125, 13){\rotatebox{90}{\color{black}\tiny{$+0.08\%$}}}
		\put(23.45, 13){\rotatebox{90}{\color{black}\tiny{$+0.55\%$}}}
		
		\put(27.2, 5.5){\rotatebox{90}{\color{white}\tiny{$5.67\%$}}}
		\put(29.1125, 5.5){\rotatebox{90}{\color{white}\tiny{$4.99\% + 0.06\%$}}}
		\put(30.95, 5.5){\rotatebox{90}{\color{white}\tiny{$5.47\% - 0.02\%$}}}
		
		% ------------------------------ %
		% +33.8
		\put(38.3, 5.5){\rotatebox{90}{\color{white}\tiny{$1.69\%$}}}
		\put(40.2125, 5.5){\rotatebox{90}{\color{white}\tiny{$1.97\% - 0.05$}}}
		\put(42.05, 5.5){\rotatebox{90}{\color{white}\tiny{$1.74\% + 0.10$}}}
		
		\put(46, 5.5){\rotatebox{90}{\color{white}\tiny{$7.15\%$}}}
		\put(47.9125, 5.5){\rotatebox{90}{\color{white}\tiny{$7.50\% + 0.03\%$}}}
		\put(49.75, 5.5){\rotatebox{90}{\color{white}\tiny{$7.50\% + 0.13\%$}}}
		
		\put(53.5, 5.5){\rotatebox{90}{\color{white}\tiny{$4.06\%$}}}
		\put(55.4125, 5.5){\rotatebox{90}{\color{white}\tiny{$3.96\% +0.47\%$}}}
		\put(57.25, 5.5){\rotatebox{90}{\color{white}\tiny{$4.00\% +0.29\%$}}}
		
		\put(61, 5.5){\rotatebox{90}{\color{white}\tiny{$5.41\%$}}}
		\put(62.9125, 5.5){\rotatebox{90}{\color{white}\tiny{$5.05\% -0.03\%$}}}
		\put(64.75, 5.5){\rotatebox{90}{\color{white}\tiny{$5.94\% -0.60\%$}}}
		
		% ------------------------------ %
		% +33.8
		\put(72.1, 7){\rotatebox{90}{\color{black}\tiny{$2.20\%$}}}
		\put(74.0125, 9){\rotatebox{90}{\color{black}\tiny{$4.40\% + 0.23\%$}}}
		\put(75.85, 13){\rotatebox{90}{\color{black}\tiny{$4.30\% + 4.96\%$}}}
		
		\put(79.8, 5.5){\rotatebox{90}{\color{white}\tiny{$5.79\%$}}}
		\put(81.7125, 5.5){\rotatebox{90}{\color{white}\tiny{$5.89\%$}}}
		\put(83.55, 5.5){\rotatebox{90}{\color{white}\tiny{$6.02\%$}}}
		
		\put(81.7125, 12){\rotatebox{90}{\color{black}\tiny{$+ 0.53\%$}}}
		\put(83.55, 12){\rotatebox{90}{\color{black}\tiny{$+ 0.12\%$}}}
		
		\put(87.3, 5.5){\rotatebox{90}{\color{white}\tiny{$5.91\%$}}}
		\put(89.2125, 9.5){\rotatebox{90}{\color{black}\tiny{$3.70\% + 0.93\%$}}}
		\put(91.05, 9.5){\rotatebox{90}{\color{black}\tiny{$4.5\% + 0.20\%$}}}
		
		\put(94.9, 5.5){\rotatebox{90}{\color{white}\tiny{$6.93\%$}}}
		\put(96.7125, 5.5){\rotatebox{90}{\color{white}\tiny{$5.95\%$}}}
		\put(98.55, 5.5){\rotatebox{90}{\color{white}\tiny{$6.26\%$}}}
		
		\put(96.7125, 11){\rotatebox{90}{\color{black}\tiny{$+ 0.17\%$}}}
		\put(98.55, 11){\rotatebox{90}{\color{black}\tiny{$+ 0.12\%$}}}
	\end{overpic}
	\caption{D-ECE results for different IoU scores (rows) and different networks (columns) using multidimensional histogram binning (HB), conditional dependent logistic calibration (LC) and beta calibration (BC). The indices denote the subsets used for calibration and D-ECE calculation: \textcircled{1}: $(\pred)$; \textcircled{2}: $(\pred, \centerx, \centery)$; \textcircled{3}: $(\pred, \width, \height)$; \textcircled{4}: $(\pred, \centerx, \centery \width, \height)$. The height of each (blue) bar denotes the D-ECE score after calibration relative to the baseline miscalibration (red dotted line) with the respective differences of using SVI (orange). We observe an almost equal calibration performance of SVI compared to the commonly used ML estimation. Note that only the scores of groups with equal index can be compared to each other since group uses a different binning scheme to evaluate the miscalibration.}
	\label{img:result:calibration}
\end{figure*} 


==> img/picp.tex <==
\begin{figure*}[t]
	\centering
	\begin{overpic}[tics=2, width=1.0\linewidth]{img/picp.png}
		% column captions
		\put(3, 44){a) Faster R-CNN on MS COCO}
		\put(39, 44){b) RetinaNet on MS COCO}
		\put(71, 44){c) Mask R-CNN on Cityscapes}
		
		% row captions
		\put(-0.5, 25){\rotatebox{90}{PICP [\%] @ IoU 0.50}}
		\put(-0.5, 2){\rotatebox{90}{PICP [\%] @ IoU 0.75}}
		
		% ------------------------------------------------------- %
		% x-axis ticks
		\put(4.75, 24.5){\rotatebox{45}{\tiny{LC}}}
		\put(7.5, 24.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(12.5, 24.5){\rotatebox{45}{\tiny{LC}}}
		\put(15.25, 24.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(20.25, 24.5){\rotatebox{45}{\tiny{LC}}}
		\put(23, 24.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(28, 24.5){\rotatebox{45}{\tiny{LC}}}
		\put(30.75, 24.5){\rotatebox{45}{\tiny{BC}}}
		
		% ------------------------------ %
		% +33.5
		\put(38.25, 24.5){\rotatebox{45}{\tiny{LC}}}
		\put(41, 24.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(46, 24.5){\rotatebox{45}{\tiny{LC}}}
		\put(48.75, 24.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(53.75, 24.5){\rotatebox{45}{\tiny{LC}}}
		\put(56.5, 24.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(61.5, 24.5){\rotatebox{45}{\tiny{LC}}}
		\put(64.25, 24.5){\rotatebox{45}{\tiny{BC}}}
		
		% ------------------------------ %
		% +33.5
		\put(71.75, 24.5){\rotatebox{45}{\tiny{LC}}}
		\put(74.5, 24.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(79.5, 24.5){\rotatebox{45}{\tiny{LC}}}
		\put(82.25, 24.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(87.25, 24.5){\rotatebox{45}{\tiny{LC}}}
		\put(90, 24.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(95, 24.5){\rotatebox{45}{\tiny{LC}}}
		\put(97.75, 24.5){\rotatebox{45}{\tiny{BC}}}
		
		% ------------------------------ %
		% ------------------------------ %
		
		\put(4.75, 1.5){\rotatebox{45}{\tiny{LC}}}
		\put(7.5, 1.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(12.5, 1.5){\rotatebox{45}{\tiny{LC}}}
		\put(15.25, 1.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(20.25, 1.5){\rotatebox{45}{\tiny{LC}}}
		\put(23, 1.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(28, 1.5){\rotatebox{45}{\tiny{LC}}}
		\put(30.75, 1.5){\rotatebox{45}{\tiny{BC}}}
		
		% ------------------------------ %
		% +33.5
		\put(38.25, 1.5){\rotatebox{45}{\tiny{LC}}}
		\put(41, 1.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(46, 1.5){\rotatebox{45}{\tiny{LC}}}
		\put(48.75, 1.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(53.75, 1.5){\rotatebox{45}{\tiny{LC}}}
		\put(56.5, 1.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(61.5, 1.5){\rotatebox{45}{\tiny{LC}}}
		\put(64.25, 1.5){\rotatebox{45}{\tiny{BC}}}
		
		% ------------------------------ %
		% +33.5
		\put(71.75, 1.5){\rotatebox{45}{\tiny{LC}}}
		\put(74.5, 1.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(79.5, 1.5){\rotatebox{45}{\tiny{LC}}}
		\put(82.25, 1.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(87.25, 1.5){\rotatebox{45}{\tiny{LC}}}
		\put(90, 1.5){\rotatebox{45}{\tiny{BC}}}
		
		\put(95, 1.5){\rotatebox{45}{\tiny{LC}}}
		\put(97.75, 1.5){\rotatebox{45}{\tiny{BC}}}
		
		% ------------------------------------------------------- %
		% y-axis ticks
		\put(1.75, 26.4){\tiny{0.0}}
		\put(1.75, 34.6){\tiny{0.5}}
		\put(1.75, 42.8){\tiny{1.0}}
		
		% ------------------------------ %
		% +33.5
		\put(35.25, 26.4){\tiny{0.0}}
		\put(35.25, 34.6){\tiny{0.5}}
		\put(35.25, 42.8){\tiny{1.0}}
		
		% ------------------------------ %
		% +33.5		
		\put(68.75, 26.4){\tiny{0.0}}
		\put(68.75, 34.6){\tiny{0.5}}
		\put(68.75, 42.8){\tiny{1.0}}
		
		% ------------------------------ %
		% ------------------------------ %
		\put(1.75, 3.4){\tiny{0.0}}
		\put(1.75, 11.6){\tiny{0.5}}
		\put(1.75, 19.8){\tiny{1.0}}
		
		% ------------------------------ %
		% +33.5
		\put(35.25, 3.4){\tiny{0.0}}
		\put(35.25, 11.6){\tiny{0.5}}
		\put(35.25, 19.8){\tiny{1.0}}
		
		% ------------------------------ %
		% +33.5
		\put(68.75, 3.4){\tiny{0.0}}
		\put(68.75, 11.6){\tiny{0.5}}
		\put(68.75, 19.8){\tiny{1.0}}
		
		% ------------------------------------------------------- %
		% grouping of calibration methods on x-axis via circled digits
		\put(6.5,23){\textbf{\tiny\circled{1}}}
		\put(14.25,23){\textbf{\tiny\circled{2}}}
		\put(22,23){\textbf{\tiny\circled{3}}}
		\put(29.75,23){\textbf{\tiny\circled{4}}}
		
		% ------------------------------ %
		% +33.5
		\put(40,23){\textbf{\tiny\circled{1}}}
		\put(47.75,23){\textbf{\tiny\circled{2}}}
		\put(55.5,23){\textbf{\tiny\circled{3}}}
		\put(63.25,23){\textbf{\tiny\circled{4}}}
		
		% ------------------------------ %
		% +33.5
		\put(73.5,23){\textbf{\tiny\circled{1}}}
		\put(81.25,23){\textbf{\tiny\circled{2}}}
		\put(89,23){\textbf{\tiny\circled{3}}}
		\put(96.75,23){\textbf{\tiny\circled{4}}}
		
		% ------------------------------ %
		% ------------------------------ %
		
		\put(6.5,0){\textbf{\tiny\circled{1}}}
		\put(14.25,0){\textbf{\tiny\circled{2}}}
		\put(22,0){\textbf{\tiny\circled{3}}}
		\put(29.75,0){\textbf{\tiny\circled{4}}}
		
		% ------------------------------ %
		% +33.5
		\put(40,0){\textbf{\tiny\circled{1}}}
		\put(47.75,0){\textbf{\tiny\circled{2}}}
		\put(55.5,0){\textbf{\tiny\circled{3}}}
		\put(63.25,0){\textbf{\tiny\circled{4}}}
		
		% ------------------------------ %
		% +33.5
		\put(73.5,0){\textbf{\tiny\circled{1}}}
		\put(81.25,0){\textbf{\tiny\circled{2}}}
		\put(89,0){\textbf{\tiny\circled{3}}}
		\put(96.75,0){\textbf{\tiny\circled{4}}}
		
	\end{overpic}
	\caption{PICP results for different IoU scores (rows), different networks (columns) and different calibration methods. The indices denote the subsets used for calibration (see Fig. \ref{img:result:calibration}). Note that only the scores of groups with equal index can be compared to each other since group uses a different binning scheme to evaluate the miscalibration. It is desirable that the PICP scores are as close as possible to the used $(1-\quantile)$ (wie genau formulieren?) (red dotted line). We observe that the prediction intervals obtained by SVI already covers the observed precision in nearly $(1-\quantile)\%$ cases, especially on higher IoU scores.}
	\label{img:result:picp}
\end{figure*} 

